Differentiable Biomechanics for Markerless Motion Capture in Upper Limb Stroke Rehabilitation: A Comparison with Optical Motion Capture

Marker-based Optical Motion Capture (OMC) paired with biomechanical modeling is currently considered the most precise and accurate method for measuring human movement kinematics. However, combining differentiable biomechanical modeling with Markerless Motion Capture (MMC) offers a promising approach to motion capture in clinical settings, requiring only minimal equipment, such as synchronized webcams, and minimal effort for data collection. This study compares key kinematic outcomes from biomechanically modeled MMC and OMC data in 15 stroke patients performing the drinking task, a functional task recommended for assessing upper limb movement quality. We observed a high level of agreement in kinematic trajectories between MMC and OMC, as indicated by high correlations (median r above 0.95 for the majority of kinematic trajectories) and median RMSE values ranging from 2-5 degrees for joint angles, 0.04 m/s for end-effector velocity, and 6 mm for trunk displacement. Trial-to-trial biases between OMC and MMC were consistent within participant sessions, with interquartile ranges of bias around 1-3 degrees for joint angles, 0.01 m/s in end-effector velocity, and approximately 3mm for trunk displacement. Our findings indicate that our MMC for arm tracking is approaching the accuracy of marker-based methods, supporting its potential for use in clinical settings. MMC could provide valuable insights into movement rehabilitation in stroke patients, potentially enhancing the effectiveness of rehabilitation strategies.

==> figures/placeholder/Overlays.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage{subcaption}  % For subfigures and subcaptions

\begin{figure}[ht]
    \centering
    % First image
    \begin{minipage}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/placeholder/overlay.png}
        \caption*{OpenSim OMC}
    \end{minipage}
    \hfill
    % Second image
    \begin{minipage}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/placeholder/overlay.png}
        \caption*{Overlay MMC1}
    \end{minipage}
    \hfill
    % Third image
    \begin{minipage}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/placeholder/overlay.png}
        \caption*{Overlay MMC2}
    \end{minipage}
    \hfill

    \caption{Placeholder Biomech. models and Overlays}
\end{figure}


==> figures/placeholder/ResultsPlaceholderKinematicsAndOverlays.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage{subcaption}  % For subfigures and subcaptions

\begin{figure*}[ht]
    \centering
    % First image
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/placeholder/Elbow Flexion.png}
        \caption*{(a) Elbow \\ F/E [°]}
    \end{minipage}
    \hfill
    % Second image
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/placeholder/Elbow Flexion.png}
        \caption*{(b) Elbow \\ v F/E [°/s]}
    \end{minipage}
    \hfill
    % Third image
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/placeholder/Elbow Flexion.png}
        \caption*{(c) Shoulder \\ F/E [°]}
    \end{minipage}
    \hfill
    % Fourth image
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/placeholder/Elbow Flexion.png}
        \caption*{(d) Shoulder \\ Ab/Ad [°]}
    \end{minipage}
    \hfill
    % Fifth image
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/placeholder/Elbow Flexion.png}
        \caption*{(e) Trunk \\ d [mm]}
    \end{minipage}
    \hfill
    % Sixth image
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/placeholder/Elbow Flexion.png}
        \caption*{(f) Endeffector \\ v [mm/s]}
    \end{minipage}
    
    \caption{Placeholder kinematics plots}
\end{figure*}


==> tables/archive/StudyPopulation_stats.tex <==
\begin{table}[H]
\begin{tabular}{@{}cccccccc@{}}
\toprule
ID master    & ID DIZH   & age & gender   & days since stroke & dominant hand & affected side & FMA-UE \\ \midrule
7            & 4         & 53  & M        & 37                & R             & R             & 49     \\
8            & 5         & 80  & F        & 192               & R             & B             & 63     \\
10           & 6         & 82  & M        & 844               & R             & L             & 57     \\
12           & 8         & 44  & M        & 1000              & R             & R             & 66     \\
13           & 9         & 87  & F        & 1613              & R             & R             & 62     \\
14           & 10        & 59  & F        & 55                & R             & L             & 64     \\
15           & 11        & 78  & M        & 1535              & R             & L             & 62     \\
17           & 12        & 45  & M        & 1665              & R             & R             & 64     \\
19           & 13        & 73  & F        & 51                & R             & R             & 43     \\
24           & 14        & 86  & M        & 173               & R             & L             & 51     \\
25           & 15        & 84  & M        & 1774              & R             & R             & 61     \\
27           & 16        & 68  & M        & 28                & R             & R             & 60     \\
28           & 17        & 87  & F        & 1337              & L             & L             & 48     \\
30           & 18        & 74  & M        & 424               & R             & R             & 39     \\
31           & 19        & 68  & F        & 88                & R             & L             & 55     \\
34           & 20        & 78  & M        & 78                & R             & R             & 28     \\ \midrule
\multicolumn{2}{c}{mean} & 72  & 10m / 6f & 680          & 1L / 15R      & 6L / 9R / 1B & 54.5  \\
\multicolumn{2}{c}{std}  & 14  &          & 694           &               &               & 10.8   \\ \bottomrule
\end{tabular}
\end{table}


